Enhancing Language Model Rationality with Bi-Directional Deliberation Reasoning

This paper introduces BI-Directional DEliberation Reasoning (BIDDER), a novel reasoning approach to enhance the decision rationality of language models. Traditional reasoning methods typically rely on historical information and employ uni-directional (left-to-right) reasoning strategy. This lack of bi-directional deliberation reasoning results in limited awareness of potential future outcomes and insufficient integration of historical context, leading to suboptimal decisions. BIDDER addresses this gap by incorporating principles of rational decision-making, specifically managing uncertainty and predicting expected utility. Our approach involves three key processes: Inferring hidden states to represent uncertain information in the decision-making process from historical data; Using these hidden states to predict future potential states and potential outcomes; Integrating historical information (past contexts) and long-term outcomes (future contexts) to inform reasoning. By leveraging bi-directional reasoning, BIDDER ensures thorough exploration of both past and future contexts, leading to more informed and rational decisions. We tested BIDDER's effectiveness in two well-defined scenarios: Poker (Limit Texas Hold'em) and Negotiation. Our experiments demonstrate that BIDDER significantly improves the decision-making capabilities of LLMs and LLM agents.

==> tabel/tab_ablation.tex <==
\begin{table}[ht]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{@{}ll|cc@{}}
\toprule
                                                         &                                  & \multicolumn{2}{c}{Limit Texas Hold'em}  \\
                                                         & Variants                          & Avg Payoff       & Rational Degree        \\ \midrule
                                                         & BIDDER                           & \textbf{1.59}             & \textbf{58.97\%} \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{Module}}             & w/o Hidden Info Inference & 1.27 ($\downarrow  0.32$)                 &  52.82 ($\downarrow  6.15\%$)       \\
\multicolumn{1}{l|}{}                                    & w/o Future Exploration           & -0.17 ($\downarrow  1.76$)                  & 8.87 ($\downarrow  50.10\%$)  \\
% \multicolumn{1}{l|}{}                                    & w/o Reward Aggregation  &                  &                       &                &                \\ \midrule
\midrule
\multicolumn{1}{l|}{\multirow{2}{*}{Aggregate Function}} & with Max                         &  1.35 ($\downarrow  0.24$)                &      57.17\% ($\downarrow  1.8\%$)  \\
\multicolumn{1}{l|}{}                                    & with Min                         &   1.47 ($\downarrow  0.12$)              &       57.37 \% ($\downarrow  1.6\%$)  \\ \bottomrule
\end{tabular}
}
    \caption{\small Ablation Study Results for Limit Texas Hold'em Poker with BIDDER Varians. Displayed at the top of the table are the impacts of different modules, and the bottom  shows the results using various aggregation functions.}
    \label{tab:ablation}
    \vspace{-4mm}
\end{table}

% \begin{table*}[ht]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ll|cc@{}}
% \toprule
%                                                          &                                  & \multicolumn{2}{c|}{Limit Texas Hold'em} & \multicolumn{2}{c}{Negotiation} \\
%                                                          & variant                          & Avg Payoff       & Rational Degree       & Avg Score      & Agree Rate     \\ \midrule
%                                                          & BIDDER                           & \textbf{1.59}             & \textbf{58.97\%}                       &                &                \\ \midrule
% \multicolumn{1}{l|}{\multirow{2}{*}{Module}}             & w/o Hidden Info Inference & 1.27 ($\downarrow  0.32$)                 &  52.82 ($\downarrow  6.15\%$)                     &                &                \\
% \multicolumn{1}{l|}{}                                    & w/o Future Exploration           & -0.17 ($\downarrow  1.59+0.17$)                  & 8.87 ($\downarrow  50.10\%$)                      &                &                \\
% % \multicolumn{1}{l|}{}                                    & w/o Reward Aggregation  &                  &                       &                &                \\ \midrule
% \midrule
% \multicolumn{1}{l|}{\multirow{2}{*}{Aggregate Function}} & with Max                         &  1.35                &      57.17\%                 &                &                \\
% \multicolumn{1}{l|}{}                                    & with Min                         &   1.47               &       57.37 \%                &                &                \\ \bottomrule
% \end{tabular}
% }
%     \caption{A figure with a caption that runs for more than one line.
%     Example image is usually available through the \texttt{mwe} package
%     without even mentioning it in the preamble.}
% \end{table*}
